Noise is an Efficient Learner for Zero-Shot Vision-Language Models

Recently, test-time adaptation has garnered attention as a method for tuning models without labeled data. The conventional modus operandi for adapting pre-trained vision-language models (VLMs) during test-time primarily focuses on tuning learnable prompts; however, this approach overlooks potential distribution shifts in the visual representations themselves. In this work, we address this limitation by introducing Test-Time Noise Tuning (TNT), a novel method for handling unpredictable shifts in the visual space. TNT leverages, for the first time, a noise adaptation strategy that optimizes learnable noise directly in the visual input space, enabling adaptive feature learning from a single test sample. We further introduce a novel approach for inter-view representation alignment by explicitly enforcing coherence in embedding distances, ensuring consistent feature representations across views. Combined with scaled logits and confident view selection at inference, TNT substantially enhances VLM generalization and calibration, achieving average gains of +7.38% on natural distributions benchmark and +0.80% on cross-dataset evaluations over zero-shot CLIP. These improvements lay a strong foundation for adaptive out-of-distribution handling.

==> algos/tnt.tex <==
% \begin{minipage}[t]{0.52\textwidth}
\begin{algorithm}[t]
\caption{PyTorch style Pseudocode for TNT}
\label{alg:tnt}
\vspace{-1.ex}
\begin{lstlisting}[style=Pytorch,escapeinside={(@}{@)}]
# image = single test image 
# model = pre-trained VLM
# eps = perturbation budget for noise
# lr = learning rate to update noise
# top_k = number of top-K views
# t = number of steps
def TNT(model, image, top_k, t):
  noise = torch.randn(image.shape)
  noise = noise.clamp(-eps,eps)
  # Get N augmented views of test image
  images = augment(image) # (N,C,H,W)
  for step in range(t)
    # Add noise to augmented views of test image 
    images = images + noise
    # Get logits and feature vectors of all views 
    logits, images_feats = model(images)
    # Get indices of top-K views 
    k_indices = confidence_filter(logits, top_k)
    # Compute entropy loss on top-K views
    loss_e = entropy(logits[k_indices])
    # Compute inter-view consistency loss
    loss_vc = vc_loss(images_feats[k_indices]) 
    loss = loss_e + loss_vc
    loss.backward()
    # Update the learnable noise
    noise = noise - torch.sign(noise.grad)*lr
    noise = noise.clamp(-eps,eps)
return noise
\end{lstlisting}
\vspace{-1.ex}
\end{algorithm}
% \end{minipage}


==> tables/dummy.tex <==
{\renewcommand{\arraystretch}{1.0}
\begin{table*}[h!]
\centering
\caption{Top-1 accuracy \% of state-of-the-art baselines, where \textbf{Average} indicates average accuracies of the Cross-Datasets Generalization. The arrow $\uparrow$ and $\downarrow$ indicate improvements and decrements compared to the CLIP method, i.e., CLIP-ViT-B/16. TNT* denotes proposed method with handcrafted prompts while TNT denotes CoOp initialized prompts. \textbf{Bold} indicates best performance, \underline{underline} indicates second-best.}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lccccccccccc}
\hline
\textbf{Dataset} & \textbf{CLIP} & \textbf{CoOp} & \textbf{TPT} & \textbf{CALIP} & \textbf{C-TPT} & \textbf{SaLS} & \textbf{RLCF} & \textbf{TNT*} & \textbf{TNT} \\
\hline
Flower102 & 67.92 & 68.82 {\scriptsize (0.90) $\uparrow$} & 68.58 {\scriptsize (0.66) $\uparrow$} & 67.64 {\scriptsize (0.28) $\downarrow$} & 70.24 {\scriptsize (2.32) $\uparrow$} & 68.66 {\scriptsize (0.74) $\uparrow$} & 68.13 {\scriptsize (0.21) $\uparrow$} & 66.26 {\scriptsize (1.66) $\downarrow$} & 68.74 {\scriptsize (0.82) $\uparrow$}  \\
DTD & 44.27 & 39.24 {\scriptsize (5.03) $\downarrow$} & 45.27 {\scriptsize (1.00) $\uparrow$} & 44.44 {\scriptsize (0.17) $\uparrow$} & 44.74 {\scriptsize (0.47) $\uparrow$} & 45.15 {\scriptsize (0.88) $\uparrow$} & 45.15 {\scriptsize (0.88) $\uparrow$} & 43.85 {\scriptsize (0.42) $\downarrow$} & 41.71 {\scriptsize (2.56) $\downarrow$}  \\
OxfordPets & 88.28 & 89.53 {\scriptsize (1.25) $\uparrow$} & 86.29 {\scriptsize (2.00) $\downarrow$} & 87.82 {\scriptsize (0.46) $\downarrow$} & 87.73 {\scriptsize (0.55) $\downarrow$} & 86.40 {\scriptsize (1.88) $\downarrow$} & 86.56 {\scriptsize (1.72) $\downarrow$} & 87.84 {\scriptsize (0.44) $\downarrow$} & \textbf{89.59} {\scriptsize (1.31) $\uparrow$}  \\
UCF & 65.21 & 68.51 {\scriptsize (3.30) $\uparrow$} & 67.62 {\scriptsize (2.41) $\uparrow$} & 64.05 {\scriptsize (1.16) $\downarrow$} & 64.37 {\scriptsize (0.84) $\downarrow$} & 67.38 {\scriptsize (2.17) $\uparrow$} & 66.96 {\scriptsize (1.75) $\uparrow$} & 67.89 {\scriptsize (2.68) $\uparrow$} & 68.81 {\scriptsize (3.60) $\uparrow$}  \\
Caltech101 & 93.39 & 90.71 {\scriptsize (2.68) $\downarrow$} & 93.35 {\scriptsize (0.04) $\uparrow$} & 93.27 {\scriptsize (0.12) $\downarrow$} & 92.41 {\scriptsize (0.98) $\downarrow$} & 93.51 {\scriptsize (0.12) $\uparrow$} & 94.04 {\scriptsize (0.65) $\uparrow$} & 93.31 {\scriptsize (0.08) $\downarrow$} & \underline{94.66} {\scriptsize (1.27) $\uparrow$}  \\
Aircraft & 23.82 & 20.01 {\scriptsize (3.81) $\downarrow$} & 22.02 {\scriptsize (1.80) $\downarrow$} & 24.12 {\scriptsize (0.30) $\uparrow$} & 23.76 {\scriptsize (0.06) $\downarrow$} & 21.93 {\scriptsize (1.89) $\downarrow$} & 21.51 {\scriptsize (2.31) $\downarrow$} & 24.54 {\scriptsize (0.72) $\uparrow$} & 20.65 {\scriptsize (3.17) $\downarrow$}  \\
EuroSAT & 42.02 & 41.78 {\scriptsize (0.24) $\downarrow$} & 42.81 {\scriptsize (0.79) $\uparrow$} & 42.27 {\scriptsize (0.25) $\uparrow$} & 36.33 {\scriptsize (5.69) $\downarrow$} & 42.53 {\scriptsize (0.51) $\uparrow$} & 45.28 {\scriptsize (3.26) $\uparrow$} & 41.99 {\scriptsize (0.03) $\downarrow$} & 44.31 {\scriptsize (2.29) $\uparrow$}  \\
StanfordCars & 65.59 & 64.74 {\scriptsize (0.85) $\downarrow$} & 66.57 {\scriptsize (0.98) $\uparrow$} & 66.50 {\scriptsize (0.91) $\uparrow$} & 64.77 {\scriptsize (0.82) $\downarrow$} & 66.73 {\scriptsize (1.14) $\uparrow$} & 65.85 {\scriptsize (0.26) $\uparrow$} & 66.93 {\scriptsize (1.34) $\uparrow$} & \underline{67.38} {\scriptsize (1.79) $\uparrow$}  \\
Food101 & 83.65 & 83.96 {\scriptsize (0.31) $\uparrow$} & 84.47 {\scriptsize (0.82) $\uparrow$} & 86.93 {\scriptsize (3.28) $\uparrow$} & 81.67 {\scriptsize (2.98) $\downarrow$} & 84.47 {\scriptsize (0.82) $\uparrow$} & 84.06 {\scriptsize (0.41) $\uparrow$} & 84.10 {\scriptsize (0.45) $\uparrow$} & \textbf{83.94} {\scriptsize (0.29) $\downarrow$} \\
SUN397 & 62.61 & 64.67 {\scriptsize (2.06) $\uparrow$} & 64.82 {\scriptsize (2.21) $\uparrow$} & 63.48 {\scriptsize (0.87) $\uparrow$} & 62.56 {\scriptsize (0.05) $\downarrow$} & 64.81 {\scriptsize (2.20) $\uparrow$} & 64.59 {\scriptsize (1.98) $\uparrow$}  & \underline{65.86} {\scriptsize (3.25) $\uparrow$} & \textbf{64.86} {\scriptsize (2.25) $\uparrow$} \\
Average & 63.48 & 63.92 {\scriptsize (0.44) $\uparrow$} & 64.02 {\scriptsize (0.54) $\uparrow$} & 63.02 {\scriptsize (0.46) $\downarrow$} & 63.07 {\scriptsize (0.41) $\downarrow$} & 64.01 {\scriptsize (0.53) $\uparrow$} & 63.83 {\scriptsize (0.35) $\uparrow$} & 64.20 {\scriptsize (0.72) $\uparrow$} & \underline{66.12} {\scriptsize (2.45) $\uparrow$}  \\
\hline
\end{tabular}
\end{table*}
}
